Tangramob: an agent-based simulation framework for validating urban smart mobility solutions

Estimating the effects of introducing a range of smart mobility solutions within an urban area is a crucial concern in urban planning. The lack of a Decision Support System (DSS) for the assessment of mobility initiatives, forces local public authorities and mobility service providers to base their decisions on guidelines derived from common heuristics and best practices. These approaches can help planners in shaping mobility solutions, but given the high number of variables to consider the effects are not guaranteed. Therefore, a solution conceived respecting the available guidelines can result in a failure in a different context. In particular, difficult aspects to consider are the interactions between different mobility services available in a given urban area, and the acceptance of a given mobility initiative by the inhabitants of the area. In order to fill this gap, we introduce Tangramob, an agent-based simulation framework capable of assessing the impacts of a Smart Mobility Initiative (SMI) within an urban area of interest. Tangramob simulates how urban traffic is expected to evolve as citizens start experiencing the newly offered traveling solutions. This allows decision makers to evaluate the efficacy of their initiatives taking into account the current urban system. In this paper we provide an overview of the simulation framework along with its design. To show the potential of Tangramob, 3 mobility initiatives are simulated and compared on the same scenario. This shows how it is possible to perform comparative experiments so as to align mobility initiatives to the user goals.

==> chapters/06_simulation/simulation.tex <==
\section{Simulation}
\label{sec:simulation}

The utility of a computational model consists in the possibility of performing simulations. In simple terms, a simulation can be seen as the model coming to life according to the configured experimental control variables. In case of an \gls{ab} model we expect agents to perform actions within the environment in which they reside so as to achieve their design objectives. One of the reasons behind our choice to adopt the \gls{ab} modelling approach lies in its ability to accurately represent real-world social dynamics with little modelling efforts. This can be easily achieved by agents with the capacity to learn from their past experience to progressively improve the quality of their decisions. Such consideration leaps over the merely reactive behaviour of traditional agents and it goes into the direction of adaptive (at least) and proactive agents. 
%
Therefore, modelling such continuously evolving behavior necessitates an iterative simulation in which commuters can try different travelling alternatives out and accumulate knowledge. 
%
\textcolor{gray}{\fra{secondo me e' ridondante, gia detto anche se meno dettagliatamente} On the other hand, as outlined in section \ref{ssec:zambonelli}, the cyclical nature of the SmartHub feedback-loop requires an iterative simulation in order to capture the \gls{ssms} concept. 
Such last observation outlines the smarthub point of view and it points out the evolution-oriented behaviour behind the smart mobility services' adaption. In effect, while commuters experiment the offered traveling opportunities leaving feedbacks along the path, smarthubs will exploit such precious information in order to improve their services. On one hand, commuters increase their knowledge so as to make better decisions during each iteration (and not necessarily for the next ones). On the other hand, every single smarthub is not designed to dynamically adapt itself during the execution of a single iteration. More precisely, a smarthub is expected to perform a replanning process at the end of each iteration, starting from the commuters' feedbacks and the current state of its smart mobility services. The output of such replanning process consists in the smarthub mobility services' adaptation and it will become effective only for the next iteration. In other words, commuters do not replan because they just keep improving during the iteration, whereas smarthubs can only improve their services at the end of the day and for the day ahead. In fact, commuters can let their \gls{kb} grow by means of a learning function (like \ref{eq:learningfunction}) which alters their perception concerning the expected performance of each smart mobility service. This process happens every time a commuter finishes a leg and computes its score (i.e. feedback) according to the traveled time and distance, $CO_2$ emissions and travel comfort. Thus, commuters increase their knowledge as well as the likelihood to make more informed and better decisions in the next future as more and more feedbacks are propagated to their corresponding \gls{kb} levels. Such methodology is perfectly in line with the \gls{rl} philosophy since the commuter is expected to learn from his past experience so as to maximize the expected income of its daily mobility decisions.
} % end gray

\subsection{A coordination infrastructure for the system}\label{ssec:zambonelli}

Now that both agents and environment have been outlined, we need to find an effective way to make our model a dynamic self-improving system. This requirement serves two major aspects, since commuters need to improve the quality of their decisions, so as to maximize the expected utility of their actions, whereas smarthubs should be able to dynamically adapt their smart mobility solutions in order to better accommodate the commuters' mobility needs. Therefore, as we can observe, SmartHub is more than a simple \gls{ab} model for performing comparative experiments. In practise, such smart mobility service adaptation together with the commuters' mobility agenda synchronization could resemble a real-case implementation of the model itself. %In effect, that is the second objective of our work and this observation would be clearer as we go through the present section.     

In order to realize such picture, the Smarthub \gls{abm} is based on the coordination architecture introduced by Sassi and Zambonelli \cite{Sassi2014}, paving the way for \gls{ssms}. In particular, as discussed in section \ref{its}, traditional \gls{its} solutions make use of advanced sensors and actuators for aligning a mobility solution to the current traffic situation. However, such systems do not exploit the possibility of "engaging smartphones, users interactions and social networking, which could instead contribute to a more integrated, powerful, and flexible approach to support urban mobility at different levels and for different needs". Therefore, the basic idea of \gls{ssms} consists in \begin{quotation} "dynamically sensing the specific mobility needs of users and dynamically check them against not only the set of actual mobility services (e.g. public buses), but also against potential mobility capabilities (e.g. a private vehicle going to a specific place) that could be turned into mobility services".\cite{Sassi2014}\end{quotation} 
\begin{figure}[!htbp]
    \centering
    \includegraphics[width = .58\linewidth]{chapters/06_formalization/pics/zambo}
    \caption{The SSMS feedback loop}
    \label{fig:zambo}
\end{figure}

Therefore, as shown in figure \ref{fig:zambo}, the \gls{ssms} architecture can be envisioned as an iterative self-regulating and self-organizing process shaped as a close feedback loop. As observable, commuters and \gls{ict} infrastructures collaborate with each other in order to achieve their mobility goals, both at an individual level and an urban level. In other words, such close interactions allow commuters to improve their traveling experience while the urban transport system es expected to become more efficient. In particular, the \gls{ssms} feedback loop can be explained in the following steps:
\begin{enumerate}
    \item \emph{Detecting mobility needs} by means of on-site sensors, commuters' smartphones, cell towers, social networks and so forth. This opens up many possibilities for dynamically understanding people mobility needs with the minimal effort.
    \item \emph{Identifying a set of matching mobility solutions} capable of satisfying such needs in a proper and timely way. When possible, the system should be able to anticipate future events so as to predict the impact of the identified mobility solutions.
    \item \emph{Coordinating the activities} of the agents involved so as to adapt the mobility services according to the commuters' satisfaction. In other words, every time a commuter uses a service he leaves a personal feedback that let the system improve. 
\end{enumerate}
%
\begin{figure}[h]
    \centering
    \includegraphics[width = .8\linewidth]{chapters/06_formalization/pics/feedbackLoop}
    \caption{The SmartHub SSMS architecture}
    \label{fig:shssms}
\end{figure}

SmartHub perfectly adheres to the \gls{ssms} architecture. In fact, the above feedback loop is organized in such a way to resemble the one proposed by Sassi and Zambonelli. 

However, in our case the system is not centralized, since all the smarthub agents are expected to collaborate with each other in order to identify the proper smart mobility services that can better satisfy the mobility needs of each commuter. In particular, the original feedback loop structure can be rewritten in terms of our steps:      
\begin{enumerate}
    \item \emph{Sensing mobility needs} by means of a smartphone mobile application that collects the commuter's mobility agenda. Such approach is known under the name of \emph{participatory sensing} and it consists in the process whereby individuals and communities use mobile phones and cloud services to collect and analyze systematic data to meet an application request out of personal or financial interest \cite{Lane2008}. In our case, each commuter agent is expected to automatically synchronize his mobility agenda with the surrounding smarthubs every time an activity is going to finishing (e.g. the commuter is leaving his workplace). %In a real-case SmartHub development, such interaction could be either triggered automatically at a given time (i.e. the commuter is unconscious about the synchronization) or manually as long as it respects a proper time restriction. By the way, our \gls{ab} model follows the automatic approach. 
    %
    \item \emph{Understanding how to satisfy those needs} according to the currently available smart mobility services as well as the urban transport system status. In this step, smarthubs need to cooperate with each other in order to arrange a list of traveling alternatives for the commuter from his current location to the actual destination. \textcolor{gray}{\fra{controllare, queste cose andrebbero dette prima}
    Such collaborative task is somehow computational demanding given that each alternative is a composition of one or more consecutive legs. For instance, the most complex alternative is composed of a first-mile \emph{origin-to-hub} segment plus a \emph{hub-to-hub} segment plus a last-mile \emph{hub-to-destination} segment. In this case, each atomic traveling segment could be performed with a bunch of smart mobility services and this gives rise to many traveling opportunities. Therefore, every smarthub has the responsibility to prepare some partial or complete traveling alternatives as well as to associate each of them with a mobility cost. By doing so, the commuter agent can choose one traveling alternative among the proposed ones, according to his own preference and experience. }
    %
    \item \emph{Enabling those mobility services} involved in the the commuters' selected traveling alternatives. In particular, once a commuter select a smart mobility alternative out of all the suggested solutions, an interaction with one or two smarthubs \fra{one or two?} is performed. 
    \textcolor{gray}{\fra{controllare, queste cose andrebbero dette prima per poter essere omesse qui}%
    Assuming that the chosen alternative includes a walk segment for reaching the $smarthub_1$ (first-mile leg) as well as a carsharing segment for getting from $smarthub_1$ to $smarthub_2$ (hub-to-hub leg) and a bikesharing segment for reaching the destination from $smarthub_2$ (last-mile leg), it is clear that some reservations are needed. Specifically, $smarthub_1$ has to reserve a carsharing vehicle whereas $smarthub_2$ needs to reserve a bicycle from its bikesharing mobility service. However, what makes the whole system intelligent is the ability of all the smarthub agents to learn from the commuters' experience.}
    % In fact, every time a commuter performs a traveling alternative he will be asked to leave a feedback for each smart mobility service involved in the alternative itself. In this way, all the smarthubs will be able to adapt their smart mobility solutions in order to increase their efficiently as well as to better satisfy the commuters' mobility needs. Therefore, the more iterations the simulation support, the more efficient the whole smarthub infrastructure will be. %In a real-case implementation this translates in a system that better performs day by day.
\end{enumerate}


\subsection{The 3-phase simulation}\label{ssec:simulation3phase}

Commuter and  Smarthub agents require an iterative simulation in order to produce accurate and proper results. On one hand, our commuter agents need to maturate a sort of perception with respect to the offered smart mobility services so as to make better informed travelling decisions during the course of the day. This behaviour is absolutely required in SmartHub, since our major objective is to approximate as much as possible the mobility behaviour of actual persons as human beings. In fact, we cannot pretend to assign each commuter with a travelling alternative in a rough manner: it is the commuter itself to choose the travelling alternative out of a set of different ones. Specifically, it is expected to exploit its past experience in order to select the travelling alternative with the highest predicted performance; as we can notice, this is the actual behaviour of human beings, and in general of every conscious organism. On the other hand, smarthub agents need to improve their smart mobility services at the end of each iteration according to the commuters' feedbacks. However, we noticed that such adapting behaviour is not always required, especially in case the experimenter aims at evaluating a static smart mobility services' configuration. Anyway, an iterative simulation is still necessary for commuters and we need to provide a valid simulation architecture in order to let the agents evolve towards their design objectives. 
\begin{figure}[!htbp]
    \centering
    \includegraphics[width = .95\linewidth]{chapters/06_formalization/pics/simulationsteps}
    \caption{SmartHub simulation steps}
    \label{fig:simulationsteps}
\end{figure}

As can be seen in figure \ref{fig:simulationsteps}, the SmartHub \gls{abm} simulation is organized into the following three sequential phases: explorative, exploitative and policy-based. Each of them involves a different number of iterations and describes a specific configuration with regard to some experimental variables. Such sequential architecture does not compromise in any way the natural agents' evolution, since it can be conceived as a tool that facilitates the \emph{on-line} model optimization. In effect, contrarily to an \emph{off-line} approach, such methodology is expected to iteratively reach an optimal solution as the simulation goes on. On the other hand, \emph{off-line} procedures solve optimization problems as a prior step, so that they can show the produced results with just a single-iteration simulation. As richly discussed so far, SmartHub follows an iterative simulation according to an \emph{on-line} optimization approach, as agents can measure the outcome of their actions so as to improve their decisions. Such process is facilitated by the three simulation phases which are described as follows.
\begin{enumerate}
    \item \textbf{Explorative phase}: smart mobility services' resources are limitless and totally free, so that commuters can experience the best ever traveling performance from such services. For instance, a carsharing service would have an infinite number of cars in order to let commuters appreciate the service in an idealistic scenario. As the name suggests, the main objective of such simulation phase consists in making the commuters explore as much as possible all the smart mobility solutions that can address their daily mobility needs. In this way, commuter agents can start populating their \gls{kb}s with optimistic scores given that the experienced smart mobility services would never be so performant in the next phases. As a consequence, the smarthub's replanning behaviour is still not active since their mobility services cannot be further improved. The explorative phase requires a variable number of iterations in order to let commuters experiment the introduced traveling opportunities.    
    %
    \item \textbf{Exploitative phase}: smart mobility services' resources are restored to their original configuration and commuters can now experience the actual performance of each new traveling solution. Therefore, smarthubs' replanning is triggered and smart mobility services are improved according to commuters' feedbacks. During this phase, a commuter agent can assign each service with a score that summarizes the actual performance of such service as it is, in order to propagate this measure into the the corresponding \gls{kb} level. Considering that smart mobility services are still free (i.e. cost per hour, cost per km and fixed costs are currently equal to zero) commuters would keep accumulating knowledge even though they now start selecting the best alternative for themselves, with no regard to their daily budget.   
    %
    \item \textbf{Policy-based phase}: similarly to the previous phase, smart mobility resources are limited and smarthubs are allowed to replan. However, the smart mobility prioritization policy discussed in section \ref{shmobilitypolicy} is now introduced so as to influence the commuters' mobility decisions. In effect, as showed in table \ref{tab:alternatives}, each proposed traveling alternative is associated with a cost, expressed in currency units or points, that is expected to mitigate commuters' preferences as they need to respect their daily mobility budget. Therefore, given that commuters' \gls{kb}s should be stable at this time, the policy-based phase requires a single iteration to complete. More precisely, every single policy-based iteration produces a plausible scenario concerning the typical day of our population and permits to assess the results of the investigated smart mobility initiative.      
\end{enumerate}

%The simulation moves forward the exploitation of the commuters’ knowledge base in order to converge towards a personal welfare, that only becomes global after the introduction of the mobility policy.


==> glossary.tex <==
%% $URL$
%% $Id$
%% Glossary term definitions
%% Note, you will need to reference them in the text after defining them

\newglossaryentry{glossary}{name=glossary, description={a place to put all the terms that confuse people}}
\newglossaryentry{ohm}{name=ohm,symbol={\ensuremath{\Omega}}, description=unit of electrical resistance}  % Do not break this with newlines!
\newglossaryentry{dissertation}{name=dissertation, description={A large pile of paper that professors use to prop up shelves.}}

\newacronym{rfid}{RFID}{Radio Frequency IDentification}

\newacronym{led}{LED}{light-emitting diodes}

\newacronym{auv}{AUV}{Autonomous Undersea Vehicle}

\newacronym{ict}{ICT}{Information and Communications Technology}

\newacronym{its}{ITS}{Intelligent Transport Systems}

\newacronym{p2p}{P2P}{peer-to-peer}

\newacronym{iot}{IoT}{Internet of Things}

\newacronym{m2m}{M2M}{Machine-to-Machine}

\newacronym{ai}{AI}{Artificial Intelligence}

\newacronym{cctv}{CCTV}{Closed Circuit Television}

\newacronym{vms}{VMS}{Video Management System}

\newacronym{wifi}{WiFi}{Wireless Fidelity}

\newacronym{vsl}{VSL}{Variable Speed Limits}

\newacronym{isa}{ISA}{Intelligent Speed Adaptation}

\newacronym{ecall}{eCALL}{Emergency Vehicle Notification system}

\newacronym{cas}{CAS}{Collision Avoidance System}

\newacronym{eea}{EEA}{European Environment Agency}

\newacronym{uk}{UK}{United Kingdom}

\newacronym{abm}{ABM}{Agent Based Model}

\newacronym{abming}{ABM}{Agent Based Modeling}

\newacronym{ab}{AB}{Agent-Based}

\newacronym{rebeca}{Rebeca}{Reactive Object Language}

\newacronym{trebeca}{TRebeca}{Timed Reactive Object Language}

\newacronym{ptrebeca}{PTRebeca}{Probabilistic Timed Rebeca}

\newacronym{lts}{LTS}{Labeled Transition System}

\newacronym{ltl}{LTL}{Linear Temporal Logic}

\newacronym{matsim}{MATSim}{Multi Agent Transport Simulation}

\newacronym{sumo}{SUMO}{Simulation of Urban MObility}

\newacronym{avcas}{AVCAS}{Ant-based Vehicle Congestion Avoidance System}

\newacronym{sidra}{SIDRA}{Signalized Intersection Design and Research Aid}

\newacronym{vtrss}{VTRSs}{Vehicle Traffic Routing Systems}

\newacronym{od}{OD}{Origin-Destination}

\newacronym{at}{AT}{Autonomous Taxicab}

\newacronym{dvrp}{DVRP}{Dynamic Vehicle Routing Problem}

\newacronym{prt}{PRT}{Personal Rapid Transit}

\newacronym{agt}{AGT}{Authomated Guideway Transit}

\newacronym{rs}{RS}{Ride Sharing}

\newacronym{sp}{SP}{Smart Parking}

\newacronym{spv}{SPV}{Single Passenger Vehicle}

\newacronym{gui}{GUI}{Graphical User Interface}

\newacronym{tide}{TIDE}{Transport Innovation Deployment for Europe}

\newacronym{dss}{DSS}{Decision Support System}

\newacronym{cae}{CAE}{Computer-Aided Design}

\newacronym{civitas}{CIVITAS}{CIty-VITAlity-Sustainability}

\newacronym{sump}{SUMP}{Sustainable Urban Mobility Plan}

\newacronym{iov}{IoV}{Internet of Vehicles}

\newacronym{istat}{ISTAT}{Istituto Nazionale di Statistica}

\newacronym{kb}{KB}{Knowledge Base}

\newacronym{ca}{CA}{Cellular Automata}

\newacronym{di}{DI}{Dependency Injector}

\newacronym{eb}{EB}{Equation Based}

\newacronym{ebm}{EBM}{Equation Based Model}

\newacronym{ebming}{EBM}{Equation Based Modeling}

\newacronym{ode}{ODE}{Ordinary Differential Equations}

\newacronym{pde}{PDE}{Partial Differential Equations}

\newacronym{mas}{MAS}{Multi Agents System}

\newacronym{ssms}{SSMS}{Smart Social Mobility Services}

\newacronym{xml}{XML}{Extensible Markup Language}

\newacronym{via}{VIA}{Visualizating MATSim Results}

\newacronym{weka}{Weka}{Waikato Environment Knowledge Analysis}

\newacronym{dtd}{DTD}{Document Type Definition}

\newacronym{fifo}{FIFO}{First In First Out}

\newacronym{awt}{AWT}{Abstract Window Toolkit}

\newacronym{gwt}{GWT}{Google Web Toolkit}

\newacronym{swt}{SWT}{Standard Widget Toolkit}

\newacronym{ajax}{AJAX}{Asynchronous JavaScript and XML}

\newacronym{jar}{JAR}{Java Archive}

\newacronym{ria}{RIA}{Rich Internet Application}

\newacronym{css}{CSS}{Cascading Style Sheets}

\newacronym{sass}{SASS}{Syntactically Awesome Style Sheets}

\newacronym{gps}{GPS}{Global Positioning System}

\newacronym{rl}{RL}{Reinforcement Learning}

\newacronym{pt}{PT}{Public Transport}

\newacronym{fb}{FB}{Feedback Base}

\newacronym{jvm}{JVM}{Java Virtual Machine}

\newacronym{smi}{SMI}{Smart Mobility Initiative}

\newacronym{ztl}{ZTL}{Zona a Traffico Limitato}

\newacronym{rmc}{RMC}{Rebeca Model Checker}

\newacronym{prism}{PRISM}{Probabilistic Symbolic  Model Checker}

\newacronym{tmdp}{TMDP}{Timed Markov Decision Process}


%% Reference manual: http://ctan.uib.no/macros/latex/contrib/glossaries/glossaries-user.pdf

%% You can also define most entries near where they are used, but this may cause problems.  See manual chapter 4.8
%% Be careful about putting entries on Chapter, Section, etc.  See manual Chapter 6.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "DEGREE-NAME-YEAR"
%%% End: 

